3D-RelNet: Joint Object and Relational Network for 3D Prediction

We propose an approach to predict the 3D shape and pose for the objects present in a scene. Existing learning based methods that pursue this goal make independent predictions per object, and do not leverage the relationships amongst them. We argue that reasoning about these relationships is crucial, and present an approach to incorporate these in a 3D prediction framework. In addition to independent per-object predictions, we predict pairwise relations in the form of relative 3D pose, and demonstrate that these can be easily incorporated to improve object level estimates. We report performance across different datasets (SUNCG, NYUv2), and show that our approach significantly improves over independent prediction approaches while also outperforming alternate implicit reasoning methods.

==> results/crf_vis.tex <==
\begin{table*}
\setlength{\tabcolsep}{0.15em} 
\centering
  \scalebox{0.95}{
\begin{tabular}{cccc@{\hskip 0.2in}cccc}
\toprule
Image & GT & Factored3D & CRF  & Image & GT & Factored3D & CRF\\ 
\midrule
\addpic{figures/crf_vis/0_img.jpg} & \addpic{figures/crf_vis/0_gt.jpg}  & \addpic{figures/crf_vis/0_baseline.jpg} & \addpic{figures/crf_vis/0_ours.jpg} &
\addpic{figures/crf_vis/1_img.jpg} & \addpic{figures/crf_vis/1_gt.jpg}  & \addpic{figures/crf_vis/1_baseline.jpg} & \addpic{figures/crf_vis/1_ours.jpg}  \\ 
\addpic{figures/crf_vis/2_img.jpg} & \addpic{figures/crf_vis/2_gt.jpg}  & \addpic{figures/crf_vis/2_baseline.jpg} & \addpic{figures/crf_vis/2_ours.jpg} & 
\addpic{figures/crf_vis/3_img.jpg} & \addpic{figures/crf_vis/3_gt.jpg}  & \addpic{figures/crf_vis/3_baseline.jpg} & \addpic{figures/crf_vis/3_ours.jpg}
 \\ 
\bottomrule 
\end{tabular}
}
\vspace{-0.1in}
\captionof{figure}{\textbf{factored3D + CRF in GT Box setting}: We visualize sample prediction results in the GT Box setting Section {\color{red} 4.2} of the main manuscript for the Factored3D + CRF model. We notice there are no significant changes to the object poses on using the CRF model.}
\label{fig:crf-gt-vis}
\end{table*} 

==> results/detectionNYU.tex <==

% \renewcommand{\arraystretch}{1.3}
% \setlength{\tabcolsep}{2pt}
\begin{table}[H]
\centering \small{
    \scalebox{1.0}{
\begin{tabular}{l |cccc}
\toprule
Method & all & box2d + trans  & box2d + rot & box2d + scale \\
\midrule
Factored3D           & 5.30 & 17.17 &  20.36 & 28.36  \\
Interaction Net & 7.57 & 19.92 & 20.39 & 30.93\\
GCN      & 6.49 & 17.39 & 21.85 & 30.42 \\
Ours               & {\bf 8.49} & {\bf 21.16}  & {\bf 22.81}  & {\bf 31.91}\\
\bottomrule
\end{tabular} }}
\vspace{-0.05in}
  \caption{We report the mean Average Precision (mAP) values for the \textbf{detection setting} for NYU. Note that the threshold for scale is different from the one used in SUNCG Table \ref{tab:detection-SUNCG}.}
  %\todo{Nilesh - I had made a "all-X" table, was this changed? If so, Sec 4.3 will also need to be written differently}
\label{tab:detection-NYU}
\end{table}

==> results/nyu.tex <==
% \begin{table}[t]
% \setlength{\tabcolsep}{0.3em} 
% \centering 
% \footnotesize{
% \scalebox{0.85}{
%   \begin{tabular}{c|ccc|ccc|ccc|ccc}
%     \toprule
%     &\multicolumn{3}{c}{Translation}
%     &\multicolumn{3}{c}{Rotation}
%     & \multicolumn{3}{c}{Scale}\\
%     \cmidrule(r){2-4}\cmidrule(l){5-7}\cmidrule(l){8-10}\cmidrule(l){11-13} 
%     Method &Median& Mean & (Err $\le 0.5$)\%   &Median& Mean & (Err $\le 30$)\%  &Median& Mean & (Err $\le 0.2$)\%\\
%     \midrule
%     Factored3D      & 0.47  & 0.59 & 53.6 & 12.87 & 39.67 & 67.6 & 0.35 & 0.37  & 21.5 \\
%     Interaction Net & 0.43 & 0.52 & 59.6 & {\bf 12.23}  & {\bf 35.86} & 69.1 & 0.32 & 0.35 & 23.1 \\
%     GCN             & 0.45 & 0.56 & 56.2 & 12.45 & 36.88 & 69.4 & 0.33 & 0.36 & 20.5 \\
%     Ours            & {\bf 0.42} & {\bf 0.51} & {\bf 60.0}   & 12.54 & 36.19 & {\bf 69.6} & {\bf 0.31} & {\bf 0.35} & {\bf 25.6}\\
%     \hline
% \end{tabular}
% }
% }
% \caption{Results on NYU. \IM{Do you see any issues?}}
% \label{tab:nyu-gt-boxes}
% \end{table}
